Regionalized models for Spanish language variations based on Twitter

Spanish is one of the most spoken languages in the globe, but not necessarily Spanish is written and spoken in the same way in different countries. Understanding local language variations can help to improve model performances on regional tasks, both understanding local structures and also improving the message's content. For instance, think about a machine learning engineer who automatizes some language classification task on a particular region or a social scientist trying to understand a regional event with echoes on social media; both can take advantage of dialect-based language models to understand what is happening with more contextual information hence more precision. This manuscript presents and describes a set of regionalized resources for the Spanish language built on four-year Twitter public messages geotagged in 26 Spanish-speaking countries. We introduce word embeddings based on FastText, language models based on BERT, and per-region sample corpora. We also provide a broad comparison among regions covering lexical and semantical similarities; as well as examples of using regional resources on message classification tasks.

==> NEW_Linguistic resources for Spanish language variations in Twitter/sn-sample-bib.tex <==
\begin{thebibliography}{29}
%% \expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
%% 
%% \bibitem[{Alessa, Faezipour, and Alhassan(2018)}]{Alessa2018}
%% Alessa, A., M.~Faezipour, and Z.~Alhassan. 2018.
%% \newblock Text classification of flu-related tweets using fasttext with
%%   sentiment and keyword features.
%% \newblock In \emph{2018 IEEE International Conference on Healthcare Informatics
%%   (ICHI)}, pages 366--367.
%% 
%% \bibitem[{Arrigo, Liberati, and Mariani(2021)}]{arrigo2021social}
%% Arrigo, Elisa, Caterina Liberati, and Paolo Mariani. 2021.
%% \newblock Social media data and users' preferences: A statistical analysis to
%%   support marketing communication.
%% \newblock \emph{Big Data Research}, 24:100189.
%% 
%% \bibitem[{Bezanson et~al.(2017)Bezanson, Edelman, Karpinski, and
%%   Shah}]{bezanson2017julia}
%% Bezanson, Jeff, Alan Edelman, Stefan Karpinski, and Viral~B Shah. 2017.
%% \newblock Julia: A fresh approach to numerical computing.
%% \newblock \emph{SIAM review}, 59(1):65--98.
%% 
%% \bibitem[{Corea(2016)}]{corea2016can}
%% Corea, Francesco. 2016.
%% \newblock Can twitter proxy the investors' sentiment? the case for the
%%   technology sector.
%% \newblock \emph{Big Data Research}, 4:70--74.
%% 

\bibitem{mcinnes2020umap}McInnes, L., Healy, J. \& Melville, J. UMAP: Uniform Manifold Approximation and Projection for Dimension Reduction.  (2020)

\bibitem{Gelbukh2001} Gelbukh, A. \& Sidorov, G. Zipf and Heaps Laws' Coefficients Depend on Language. {\em Computational Linguistics And Intelligent Text Processing}. pp. 332-335 (2001)

\bibitem{schutze2008introduction}Schütze, H., Manning, C. \& Raghavan, P. Introduction to information retrieval. Cambridge University Press Cambridge. (2008).

\bibitem{jimenez2018automatic}Jimenez, S., Dueñas, G., Gelbukh, A., Rodriguez-Diaz, C. \& Mancera, S. Automatic detection of regional words for pan-hispanic spanish on twitter. {\em Ibero-American Conference On Artificial Intelligence}. pp. 404-416 (2018)

\bibitem{li2019empirical}Li, M., Chng, E., Chong, A. \& See, S. An empirical analysis of emoji usage on Twitter. {\em Industrial Management \& Data Systems}. (2019)

\bibitem{huertas2022bertuit}Huertas-Tato, J., Martin, A. \& Camacho, D. BERTuit: Understanding Spanish language in Twitter through a native transformer. {\em ArXiv Preprint ArXiv:2204.03465}. (2022)

\bibitem{hong2011language}Hong, L., Convertino, G. \& Chi, E. Language matters in twitter: A large scale study. {\em Proceedings Of The International AAAI Conference On Web And Social Media}. \textbf{5}, 518-521 (2011)

\bibitem{park2013emoticon}Park, J., Barash, V., Fink, C. \& Cha, M. Emoticon style: Interpreting differences in emoticons across cultures. {\em Proceedings Of The International AAAI Conference On Web And Social Media}. \textbf{7}, 466-475 (2013)

\bibitem{alshutayri2017exploring}Alshutayri, A. \& Atwell, E. Exploring Twitter as a source of an Arabic dialect corpus. {\em International Journal Of Computational Linguistics (IJCL)}. \textbf{8}, 37-44 (2017)

\bibitem{lamontagne2022phonological}Lamontagne, J. \& McCulloch, G. Phonological variation on Twitter: Evidence from letter repetition in three French dialects. {\em Journal Of French Language Studies}. pp. 1-32 (2022)

\bibitem[{Hovy et~al.(2020) Hovy, Dirk and Rahimi, Afshin and Baldwin, Timothy and Brooke, Julian}]{hovy2020visualizing}
 Hovy, Dirk and Rahimi, Afshin and Baldwin, Timothy and Brooke, Julian. 2020.
 \newblock Visualizing regional language variation across Europe on Twitter
 \newblock \emph{Handbook of the Changing World Language Map},
  3719--3742

\bibitem[{Hoff (2020) Hoff, Mark}]{hoff2020cerca}
 Hoff, Mark. 2020.
 \newblock Cerca m{\'\i}o/a or cerca de m{\'\i}? A variationist analysis of Spanish locative+ possessive on Twitter.
 \newblock \emph{Studies in Hispanic and Lusophone Linguistics},
  51--78.
   
\bibitem[{Crampton et~al.(2013)Crampton, Graham, Poorthuis, Shelton, Stephens,
   Wilson, and Zook}]{CR2013}
 Crampton, Jeremy~W., Mark Graham, Ate Poorthuis, Taylor Shelton, Monica
   Stephens, Matthew~W. Wilson, and Matthew Zook. 2013.
 \newblock Beyond the geotag: situating "big data" and leveraging the potential
   of the geoweb.
 \newblock \emph{Cartography and Geographic Information Science},
   40(2):130--139.
%% 
%% \bibitem[{De~Sarkar, Yang, and Mukherjee(2018)}]{C181285}
%% De~Sarkar, Sohan, Fan Yang, and Arjun Mukherjee. 2018.
%% \newblock Attending sentences to detect satirical fake news.
%% \newblock In \emph{Proceedings of the 27th International Conference on
%%   Computational Linguistics}, pages 3371--3380, Association for Computational
%%   Linguistics.
%% 
 \bibitem[{Devlin et~al.(2019)Devlin, Chang, Lee, and Toutanova}]{devlin-etal-2019-bert}
 Devlin, Jacob, Chang, Ming-Wei, Lee, Kenton and Toutanova, Kristina. 2019
 \newblock {BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding
 \newblock \emph{Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)}, pages 4171--4186, Association for Computational Linguistics

%% 
\bibitem[{Donoso and S{\'a}nchez(2017)}]{Donoso2017DialectometricAO}
 Donoso, Gonzalo and David S{\'a}nchez. 2017.
 \newblock Dialectometric analysis of language variation in {T}witter.
 \newblock In \emph{Proceedings of the Fourth Workshop on {NLP} for Similar
   Languages, Varieties and Dialects ({V}ar{D}ial)}, pages 16--25, Association
   for Computational Linguistics, Valencia, Spain.
%% 
 \bibitem[{Dresner and Herring(2010)}]{dresner2010functions}
 Dresner, Eli and Susan~C Herring. 2010.
 \newblock Functions of the nonverbal in cmc: Emoticons and illocutionary force.
 \newblock \emph{Communication theory}, 20(3):249--268.
%% 
%% \bibitem[{Dunn(2019)}]{dunn2019global}
%% Dunn, Jonathan. 2019.
%% \newblock Global syntactic variation in seven languages: Toward a computational
%%   dialectology.
%% \newblock \emph{Frontiers in artificial intelligence}, 2:15.
%% 
%% \bibitem[{Dunn(2020)}]{dunn2020mapping}
%% Dunn, Jonathan. 2020.
%% \newblock Mapping languages: The corpus of global language use.
%% \newblock \emph{Language Resources and Evaluation}, 54(4):999--1018.
%% 
 \bibitem[{Gon{\c{c}}alves and S{\'a}nchez(2014)}]{gonccalves2014crowdsourcing}
 Gon{\c{c}}alves, Bruno and David S{\'a}nchez. 2014.
 \newblock Crowdsourcing dialect characterization through twitter.
 \newblock \emph{PloS one}, 9(11):e112074.
%% 
 \bibitem[{Graham, Hale, and Gaffney(2014)}]{graham2014world}
 Graham, Mark, Scott~A Hale, and Devin Gaffney. 2014.
 \newblock Where in the world are you? geolocation and language identification
   in twitter.
 \newblock \emph{The Professional Geographer}, 66(4):568--578.
%% 
%% \bibitem[{Hovy et~al.(2020)Hovy, Rahimi, Baldwin, and
%%   Brooke}]{hovy2020visualizing}
%% Hovy, Dirk, Afshin Rahimi, Timothy Baldwin, and Julian Brooke. 2020.
%% \newblock Visualizing regional language variation across europe on twitter.
%% \newblock \emph{Handbook of the Changing World Language Map}, pages 3719--3742.
%% 
 \bibitem[{Huang et~al.(2016)Huang, Guo, Kasakoff, and
   Grieve}]{huang2016understanding}
 Huang, Yuan, Diansheng Guo, Alice Kasakoff, and Jack Grieve. 2016.
 \newblock Understanding us regional linguistic variation with twitter data
   analysis.
 \newblock \emph{Computers, environment and urban systems}, 59:244--255.
%% 
 \bibitem[{Joulin et~al.(2017)Joulin, Grave, Bojanowski, and
   Mikolov}]{joulin2017bag}
 Joulin, Armand, Edouard Grave, Piotr Bojanowski, and Tomas Mikolov. 2017.
 \newblock Bag of tricks for efficient text classification.
 \newblock In \emph{Proceedings of the 15th Conference of the European Chapter
   of the Association for Computational Linguistics: Volume 2, Short Papers},
   pages 427--431, Association for Computational Linguistics.
%% 
%% \bibitem[{Karpathy and Fei-Fei(2015)}]{Karpathy2015CVPR}
%% Karpathy, Andrej and Li~Fei-Fei. 2015.
%% \newblock Deep visual-semantic alignments for generating image descriptions.
%% \newblock In \emph{Proceedings of the IEEE conference on computer vision and
%%   pattern recognition}, pages 3128--3137.
%% 
 \bibitem[{Kejriwal et~al.(2021)Kejriwal, Wang, Li, and
   Wang}]{kejriwal2021empirical}
 Kejriwal, Mayank, Qile Wang, Hongyu Li, and Lu~Wang. 2021.
 \newblock An empirical study of emoji usage on twitter in linguistic and
   national contexts.
 \newblock \emph{Online Social Networks and Media}, 24:100149.
%% 
%% \bibitem[{Li, Naacke, and Amann(2021)}]{li2021analytic}
%% Li, Ke, Hubert Naacke, and Bernd Amann. 2021.
%% \newblock An analytic graph data model and query language for exploring the
%%   evolution of science.
%% \newblock \emph{Big Data Research}, 26:100247.
%% 

 
%% \bibitem[{McInnes, Healy, and Melville(2020)}]{mcinnes2020umap}
%% McInnes, Leland, John Healy, and James Melville. 2020.
%% \newblock Umap: Uniform manifold approximation and projection for dimension
%%   reduction.
%% 
 \bibitem[{Mikolov et~al.(2013{\natexlab{a}})Mikolov, Sutskever, Chen, Corrado,
   and Dean}]{Mikolov2013}
 Mikolov, Tomas, Ilya Sutskever, Kai Chen, Greg Corrado, and Jeffrey Dean.
   2013{\natexlab{a}}.
 \newblock Distributed representations of words and phrases and their
   compositionality.
 \newblock In \emph{Proceedings of the 26th International Conference on Neural
   Information Processing Systems - Volume 2}, NIPS'13, pages 3111--3119, Curran
   Associates Inc., USA.
%% 
%% \bibitem[{Mikolov et~al.(2013{\natexlab{b}})Mikolov, Sutskever, Chen, Corrado,
%%   and Dean}]{fastText2013}
%% Mikolov, Tomas, Ilya Sutskever, Kai Chen, Greg~S Corrado, and Jeff Dean.
%%   2013{\natexlab{b}}.
%% \newblock Distributed representations of words and phrases and their
%%   compositionality.
%% \newblock In \emph{Advances in neural information processing systems}, pages
%%   3111--3119.
%% 
\bibitem[{Mocanu et~al.(2013)Mocanu, Baronchelli, Perra, Gon{\c{c}}alves,
   Zhang, and Vespignani}]{mocanu2013twitter}
 Mocanu, Delia, Andrea Baronchelli, Nicola Perra, Bruno Gon{\c{c}}alves, Qian
   Zhang, and Alessandro Vespignani. 2013.
 \newblock The twitter of babel: Mapping world languages through microblogging
   platforms.
 \newblock \emph{PloS one}, 8(4):e61981.
%% 
%% \bibitem[{Mohammad and Turney(2010)}]{mohammad2010}
%% Mohammad, Saif and Peter Turney. 2010.
%% \newblock Emotions evoked by common words and phrases: Using {M}echanical
%%   {T}urk to create an emotion lexicon.
%% \newblock In \emph{Proceedings of the {NAACL} {HLT} 2010 Workshop on
%%   Computational Approaches to Analysis and Generation of Emotion in Text},
%%   pages 26--34, Association for Computational Linguistics, Los Angeles, CA.
%% 
%% \bibitem[{Mohammad and Turney(2013)}]{Mohammad13}
%% Mohammad, Saif~M. and Peter~D. Turney. 2013.
%% \newblock Crowdsourcing a word-emotion association lexicon.
%% \newblock \emph{Computational Intelligence}, 29(3):436--465.
%% 
\bibitem{wada2018unsupervised}Wada, T. \& Iwata, T. Unsupervised Cross-lingual Word Embedding by Multilingual Neural Language Models. {\em CoRR}. \textbf{abs/1809.02306} (2018)
\bibitem{anowar2021dimension}Anowar, F., Sadaoui, S. \& Selim, B. Conceptual and empirical comparison of dimensionality reduction algorithms (PCA, KPCA, LDA, MDS, SVD, LLE, ISOMAP, LE, ICA, t-SNE). {\em Computer Science Review}. \textbf{40} pp. 100378 (2021)

\bibitem{mikolov2013distributed} Mikolov, T., Sutskever, I., Chen, K., Corrado, G. \& Dean, J. Distributed representations of words and phrases and their compositionality. {\em Advances In Neural Information Processing Systems}. \textbf{26} (2013)

\bibitem{cotton1988spanish}Cotton, E. \& Sharp, J. Spanish in the Americas. (Georgetown University Press,1988)

\bibitem{bojanowski2017enriching}Bojanowski, P., Grave, E., Joulin, A. \& Mikolov, T. Enriching word vectors with subword information. {\em Transactions Of The Association For Computational Linguistics}. \textbf{5} pp. 135-146 (2017)

\bibitem{penny2000variation}Penny, R., Penny, R. \& Ralph, P. Variation and change in Spanish. (Cambridge University Press,2000)
 \bibitem[{Pennington, Socher, and Manning(2014)}]{glove}
 Pennington, Jeffrey, Richard Socher, and Christopher~D Manning. 2014.
 \newblock Glove: Global vectors for word representation.
 \newblock In \emph{Proceedings of the 2014 conference on empirical methods in
   natural language processing (EMNLP)}, pages 1532--1543.
%% 
 \bibitem[{Peters et~al..(2018)Peters, Neumann, Iyyer, Gardner, Clark, Lee, and Zettlemoyer}]{peters-etal-2018-deep}
 Peters, Matthew E. and Neumann, Mark and Iyyer, Mohit and Gardner, Matt and Clark, Christopher and Lee, Kenton and Zettlemoyer, Luke. 2018
 \newblock Deep Contextualized Word Representations
 \newblock \emph{Proceedings of the 2018 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long Papers)}, pages 2227--2237, Association for Computational Linguistics
%% 
\bibitem[{Rodriguez-Diaz et~al.(2018)Rodriguez-Diaz, Jimenez, Due{\~n}as,
   Bonilla, and Gelbukh}]{rodriguez2018dialectones}
   Rodriguez-Diaz, Carlos~A, Sergio Jimenez, George Due{\~n}as, Johnatan~Estiven
  Bonilla, and Alexander Gelbukh. 2018.
 \newblock Dialectones: Finding statistically significant dialectal boundaries
   using twitter data.
   \newblock \emph{Computaci{\'o}n y Sistemas}, 22(4):1213--1222.
%% 
%% \bibitem[{Wan et~al.(2018)Wan, Li, Zhang, Wang, and Li}]{Shuo2018}
%% Wan, Shuo, Bohan Li, Anman Zhang, Kai Wang, and Xue Li. 2018.
%% \newblock Vertical and sequential sentiment analysis of micro-blog topic.
%% \newblock In \emph{Advanced Data Mining and Applications}, pages 353--363,
%%   Springer International Publishing, Cham.
%% 
 \bibitem[{Yang, Macdonald, and Ounis(2018)}]{Yang2018}
 Yang, Xiao, Craig Macdonald, and Iadh Ounis. 2018.
 \newblock Using word embeddings in twitter election classification.
 \newblock \emph{Information Retrieval Journal}, 21(2):183--207.
%% 
 \bibitem[{Grave, Edouard and Bojanowski, Piotr and Gupta, Prakhar and Joulin, Armand and Mikolov, Tomas}]{grave2018learning}
 Edouard Grave, Piotr Bojanowski, Prakhar Gupta, Armand Joulin, and Tomas Mikolov. 2018. 
   \newblock Learning Word Vectors for 157 Languages.
   \newblock \emph{Proceedings of the International Conference on Language Resources and Evaluation (LREC 2018)}
%% 
%% 
%% \bibitem[{Cañete, José}]{Canete2019}
%% José Cañete. 2019. 
%%   \newblock Compilation of Open Large Spanish Unannotated Corpora with some post processing.
%%   \newblock \emph{\url{https://github.com/josecannete/spanish-corpora}}
%%   \newblock [Access: 2 March 2022]
%%   
%%   \bibitem[{Cañete, José}]{CaneteEmbeddings2019}
%% José Cañete. 2019. 
%%   \newblock Spanish Word Embeddigs on the Spanish Unannotated Corpora.
%%   \newblock \emph{\url{https://github.com/BotCenter/spanishWordEmbeddings}}
%%   \newblock [Access: 2 March 2022]
%%   
%%   \bibitem[{Cardellino, Cristian}]{CardellinoEmbeddings2019}
%% Cristian Cardellino. 2019. 
%%   \newblock Spanish {B}illion {W}ords {C}orpus and {E}mbeddings.
%%   \newblock \emph{\url{https://crscardellino.github.io/SBWCE/}}
%%   \newblock [Access: 2 March 2022]
%%   
%% 
%% 
\bibitem{frenda2019online}Frenda, S., Ghanem, B., Gómez, M. \& Rosso, P. Online hate speech against women: Automatic identification of misogyny and sexism on twitter. {\em Journal Of Intelligent \& Fuzzy Systems}. \textbf{36}, 4743-4752 (2019)

\bibitem{vashisth2020gender}Vashisth, P. \& Meehan, K. Gender classification using twitter text data. {\em 2020 31st Irish Signals And Systems Conference (ISSC)}. pp. 1-6 (2020)

\bibitem{mooney2009evaluating}Mooney, P., Winstanley, A. \& Corcoran, P. Evaluating Twitter for use in environmental awareness campaigns. (Dept. of Computer Science, National University of Ireland, Maynooth,2009)
\bibitem{suhasini2020emotion}Suhasini, M. \& Srinivasu, B. Emotion detection framework for twitter data using supervised classifiers. {\em Data Engineering And Communication Technology}. pp. 565-576 (2020)

\bibitem{paul2011you}Paul, M. \& Dredze, M. You are what you tweet: Analyzing twitter for public health. {\em Proceedings Of The International AAAI Conference On Web And Social Media}. \textbf{5}, 265-272 (2011)

\bibitem{finfgeld2015twitter}Finfgeld-Connett, D. Twitter and health science research. {\em Western Journal Of Nursing Research}. \textbf{37}, 1269-1283 (2015)

 \bibitem[{CKennedy, Brendan et al. (2022)}]{kennedy2022introducing}
 CKennedy, Brendan and Atari, Mohammad and Davani, Aida Mostafazadeh and Yeh, Leigh and Omrani, Ali and Kim, Yehsong and Coombs, Kris and Havaldar, Shreya and Portillo-Wightman, Gwenyth and Gonzalez, Elaine and others (2022).
   \newblock Introducing the Gab Hate Corpus: defining and applying hate-based rhetoric to social media posts at scale.
   \newblock \emph{Language Resources and Evaluation}, Springer.
%%   
%%   
%%  
 \bibitem[{Escudero-Mancebo, David and Corrales-Astorgano, Mario and Carde{\~n}oso-Payo, Valent{\'\i}n and Aguilar, Lourdes and Gonz{\'a}lez-Ferreras, C{\'e}sar and Mart{\'\i}nez-Castilla, Pastora and Flores-Lucas, Valle (2022)}]{escudero2022prautocal}
 Escudero-Mancebo, David and Corrales-Astorgano, Mario and Carde{\~n}oso-Payo, Valent{\'\i}n and Aguilar, Lourdes and Gonz{\'a}lez-Ferreras, C{\'e}sar and Mart{\'\i}nez-Castilla, Pastora and Flores-Lucas, Valle. 2022.
 \newblock Prautocal corpus: A corpus for the study of down syndrome prosodic aspects
 \newblock Language Resources and Evaluation, Springer.
%% 
   \bibitem[{Gruszczy{\'n}ski, W{\l}odzimierz and Adamiec, Dorota and Bronikowska, Renata and Kiera{\'s}, Witold and Modrzejewski, Emanuel and Wieczorek, Aleksandra and Woli{\'n}ski, Marcin (2022)}]{gruszczynski2022electronic}
 Gruszczy{\'n}ski, W{\l}odzimierz and Adamiec, Dorota and Bronikowska, Renata and Kiera{\'s}, Witold and Modrzejewski, Emanuel and Wieczorek, Aleksandra and Woli{\'n}ski, Marcin, 2022.
 \newblock The Electronic Corpus of 17th-and 18th-century Polish Texts
 \newblock Language Resources and Evaluation, Springer.
%%   
%%   
%% 
\end{thebibliography}

